The track-length extension fitting algorithm for energy measurement of interacting particles in liquid argon TPCs and its performance with ProtoDUNE-SP data

This paper introduces a novel track-length extension fitting algorithm for measuring the kinetic energies of inelastically interacting particles in liquid argon time projection chambers (LArTPCs). The algorithm finds the most probable offset in track length for a track-like object by comparing the measured ionization density as a function of position with a theoretical prediction of the energy loss as a function of the energy, including models of electron recombination and detector response. The algorithm can be used to measure the energies of particles that interact before they stop, such as charged pions that are absorbed by argon nuclei. The algorithm's energy measurement resolutions and fractional biases are presented as functions of particle kinetic energy and number of track hits using samples of stopping secondary charged pions in data collected by the ProtoDUNE-SP detector, and also in a detailed simulation. Additional studies describe the impact of the dE/dx model on energy measurement performance. The method described in this paper to characterize the energy measurement performance can be repeated in any LArTPC experiment using stopping secondary charged pions.

==> export_xml_authors_2024-08-11_arxiv.tex <==
# Plain-text author list (see https://arxiv.org/help/prep) produced at 2024-08-11, from master list generated at 2024-08-11
DUNE Collaboration: A. Abed Abud, B. Abi, R. Acciarri, M. A. Acero, M. R. Adames, G. Adamov, M. Adamowski, D. Adams, M. Adinolfi, C. Adriano, A. Aduszkiewicz, J. Aguilar, F. Akbar, N. S. Alex, K. Allison, S. Alonso Monsalve, M. Alrashed, A. Alton, R. Alvarez, T. Alves, H. Amar, P. Amedo, J. Anderson, C. Andreopoulos, M. Andreotti, M. P. Andrews, F. Andrianala, S. Andringa, N. Anfimov, A. Ankowski, D. Antic, M. Antoniassi, M. Antonova, A. Antoshkin, A. Aranda-Fernandez, L. Arellano, E. Arrieta Diaz, M. A. Arroyave, J. Asaadi, A. Ashkenazi, D. Asner, L. Asquith, E. Atkin, D. Auguste, A. Aurisano, V. Aushev, D. Autiero, M. B. Azam, F. Azfar, A. Back, H. Back, J. J. Back, I. Bagaturia, L. Bagby, N. Balashov, S. Balasubramanian, P. Baldi, W. Baldini, J. Baldonedo, B. Baller, B. Bambah, R. Banerjee, F. Barao, D. Barbu, G. Barenboim, P.\ Barham~Alz\'as, G. J. Barker, W. Barkhouse, G. Barr, J. Barranco Monarca, A. Barros, N. Barros, D. Barrow, J. L. Barrow, A. Basharina-Freshville, A. Bashyal, V. Basque, C. Batchelor, L. Bathe-Peters, J.B.R. Battat, F. Battisti, F. Bay, M. C. Q. Bazetto, J. L. L. Bazo Alba, J. F. Beacom, E. Bechetoille, B. Behera, E. Belchior, G. Bell, L. Bellantoni, G. Bellettini, V. Bellini, O. Beltramello, N. Benekos, C. Benitez Montiel, D. Benjamin, F. Bento Neves, J. Berger, S. Berkman, J. Bernal, P. Bernardini, A. Bersani, S. Bertolucci, M. Betancourt, A. Betancur Rodr\'iguez, A. Bevan, Y. Bezawada, A. T. Bezerra, T. J. Bezerra, A. Bhat, V. Bhatnagar, J. Bhatt, M. Bhattacharjee, M. Bhattacharya, S. Bhuller, B. Bhuyan, S. Biagi, J. Bian, K. Biery, B. Bilki, M. Bishai, A. Bitadze, A. Blake, F. D. Blaszczyk, G. C. Blazey, E. Blucher, A. Bodek, J. Bogenschuetz, J. Boissevain, S. Bolognesi, T. Bolton, L. Bomben, M. Bonesini, C. Bonilla-Diaz, F. Bonini, A. Booth, F. Boran, S. Bordoni, R. Borges Merlo, A. Borkum, N. Bostan, R. Bouet, J. Boza, J. Bracinik, B. Brahma, D. Brailsford, F. Bramati, A. Branca, A. Brandt, J. Bremer, C. Brew, S. J. Brice, V. Brio, C. Brizzolari, C. Bromberg, J. Brooke, A. Bross, G. Brunetti, M. Brunetti, N. Buchanan, H. Budd, J. Buergi, A. Bundock, D. Burgardt, S. Butchart, G. Caceres V., I. Cagnoli, T. Cai, R. Calabrese, R. Calabrese, J. Calcutt, L. Calivers, E. Calvo, A. Caminata, A. F. Camino, W. Campanelli, A. Campani, A. Campos Benitez, N. Canci, J. Cap{\'o}, I. Caracas, D. Caratelli, D. Carber, J. M. Carceller, G. Carini, B. Carlus, M. F. Carneiro, P. Carniti, I. Caro Terrazas, H. Carranza, N. Carrara, L. Carroll, T. Carroll, A. Carter, E. Casarejos, D. Casazza, J. F. Casta{\~n}o Forero, F. A. Casta{\~n}o, A. Castillo, C. Castromonte, E. Catano-Mur, C. Cattadori, F. Cavalier, F. Cavanna, S. Centro, G. Cerati, C. Cerna, A. Cervelli, A. Cervera Villanueva, K. Chakraborty, M. Chalifour, A. Chappell, N. Charitonidis, A. Chatterjee, H. Chen, M. Chen, W. C. Chen, Y. Chen, Z. Chen-Wishart, D. Cherdack, C. Chi, F. Chiapponi, R. Chirco, N. Chitirasreemadam, K. Cho, S. Choate, G. Choi, D. Chokheli, P. S. Chong, B. Chowdhury, D. Christian, A. Chukanov, M. Chung, E. Church, M. F. Cicala, M. Cicerchia, V. Cicero, R. Ciolini, P. Clarke, G. Cline, T. E. Coan, A. G. Cocco, J. A. B. Coelho, A. Cohen, J. Collazo, J. Collot, E. Conley, J. M. Conrad, M. Convery, S. Copello, P. Cova, C. Cox, L. Cremaldi, L. Cremonesi, J. I. Crespo-Anad\'on, M. Crisler, E. Cristaldo, J. Crnkovic, G. Crone, R. Cross, A. Cudd, C. Cuesta, Y. Cui, F. Curciarello, D. Cussans, J. Dai, O. Dalager, R. Dallavalle, W. Dallaway, R. D'Amico, H. da Motta, Z. A. Dar, R. Darby, L. Da Silva Peres, Q. David, G. S. Davies, S. Davini, J. Dawson, R. De Aguiar, P. De Almeida, P. Debbins, I. De Bonis, M. P. Decowski, A. de Gouv\^ea, P. C. De Holanda, I. L. De Icaza Astiz, P. De Jong, P. Del Amo Sanchez, A. De la Torre, G. De Lauretis, A. Delbart, D. Delepine, M. Delgado, A. Dell'Acqua, G. Delle Monache, N. Delmonte, P. De Lurgio, R. Demario, G. De Matteis, J. R. T. de Mello Neto, D. M. DeMuth, S. Dennis, C. Densham, P. Denton, G. W. Deptuch, A. De Roeck, V. De Romeri, J. P. Detje, J. Devine, R. Dharmapalan, M. Dias, A. Diaz, J. S. D\'iaz, F. D{\'\i}az, F. Di Capua, A. Di Domenico, S. Di Domizio, S. Di Falco, L. Di Giulio, P. Ding, L. Di Noto, E. Diociaiuti, C. Distefano, R. Diurba, M. Diwan, Z. Djurcic, D. Doering, S. Dolan, F. Dolek, M. J. Dolinski, D. Domenici, L. Domine, S. Donati, Y. Donon, S. Doran, D. Douglas, T.A. Doyle, A. Dragone, F. Drielsma, L. Duarte, D. Duchesneau, K. Duffy, K. Dugas, P. Dunne, B. Dutta, H. Duyang, D. A. Dwyer, A. S. Dyshkant, S. Dytman, M. Eads, A. Earle, S. Edayath, D. Edmunds, J. Eisch, P. Englezos, A. Ereditato, T. Erjavec, C. O. Escobar, J. J. Evans, E. Ewart, A. C. Ezeribe, K. Fahey, L. Fajt, A. Falcone, M. Fani', C. Farnese, S. Farrell, Y. Farzan, D. Fedoseev, J. Felix, Y. Feng, E. Fernandez-Martinez, G. Ferry, E. Fialova, L. Fields, P. Filip, A. Filkins, F. Filthaut, R. Fine, G. Fiorillo, M. Fiorini, S. Fogarty, W. Foreman, J. Fowler, J. Franc, K. Francis, D. Franco, J. Franklin, J. Freeman, J. Fried, A. Friedland, S. Fuess, I. K. Furic, K. Furman, A. P. Furmanski, R. Gaba, A. Gabrielli, A. M~Gago, F. Galizzi, H. Gallagher, N. Gallice, V. Galymov, E. Gamberini, T. Gamble, F. Ganacim, R. Gandhi, S. Ganguly, F. Gao, S. Gao, D. Garcia-Gamez, M. \'A. Garc\'ia-Peris, F. Gardim, S. Gardiner, D. Gastler, A. Gauch, J. Gauvreau, P. Gauzzi, S. Gazzana, G. Ge, N. Geffroy, B. Gelli, S. Gent, L. Gerlach, Z. Ghorbani-Moghaddam, T. Giammaria, D. Gibin, I. Gil-Botella, S. Gilligan, A. Gioiosa, S. Giovannella, C. Girerd, A. K. Giri, C. Giugliano, V. Giusti, D. Gnani, O. Gogota, S. Gollapinni, K. Gollwitzer, R. A. Gomes, L. V. Gomez Bermeo, L. S. Gomez Fajardo, F. Gonnella, D. Gonzalez-Diaz, M. Gonzalez-Lopez, M. C. Goodman, S. Goswami, C. Gotti, J. Goudeau, E. Goudzovski, C. Grace, E. Gramellini, R. Gran, E. Granados, P. Granger, C. Grant, D. R. Gratieri, G. Grauso, P. Green, S. Greenberg, J. Greer, W. C. Griffith, F. T. Groetschla, K. Grzelak, L. Gu, W. Gu, V. Guarino, M. Guarise, R. Guenette, M. Guerzoni, D. Guffanti, A. Guglielmi, B. Guo, F. Y. Guo, A. Gupta, V. Gupta, G. Gurung, D. Gutierrez, P. Guzowski, M. M. Guzzo, S. Gwon, A. Habig, H. Hadavand, L. Haegel, R. Haenni, L. Hagaman, A. Hahn, J. Haiston, J. Hakenm\"uller, T. Hamernik, P. Hamilton, J. Hancock, F. Happacher, D. A. Harris, A.~L.~Hart, J. Hartnell, T. Hartnett, J. Harton, T. Hasegawa, C. M. Hasnip, R. Hatcher, K. Hayrapetyan, J. Hays, E. Hazen, M. He, A. Heavey, K. M. Heeger, J. Heise, P. Hellmuth, S. Henry, K. Herner, V. Hewes, A. Higuera, C. Hilgenberg, S. J. Hillier, A. Himmel, E. Hinkle, L.R. Hirsch, J. Ho, J. Hoff, A. Holin, T. Holvey, E. Hoppe, S. Horiuchi, G. A. Horton-Smith, T. Houdy, B. Howard, R. Howell, I. Hristova, M. S. Hronek, J. Huang, R.G. Huang, Z. Hulcher, M. Ibrahim, G. Iles, N. Ilic, A. M. Iliescu, R. Illingworth, G. Ingratta, A. Ioannisian, B. Irwin, L. Isenhower, M. Ismerio Oliveira, R. Itay, C.M. Jackson, V. Jain, E. James, W. Jang, B. Jargowsky, D. Jena, I. Jentz, X. Ji, C. Jiang, J. Jiang, L. Jiang, A. Jipa, J. H. Jo, F. R. Joaquim, W. Johnson, C. Jollet, B. Jones, R. Jones, N. Jovancevic, M. Judah, C. K. Jung, K. Y. Jung, T. Junk, Y. Jwa, M. Kabirnezhad, A. C. Kaboth, I. Kadenko, I. Kakorin, A. Kalitkina, D. Kalra, M. Kandemir, D. M. Kaplan, G. Karagiorgi, G. Karaman, A. Karcher, Y. Karyotakis, S. Kasai, S. P. Kasetti, L. Kashur, I. Katsioulas, A. Kauther, N. Kazaryan, L. Ke, E. Kearns, P.T. Keener, K.J. Kelly, E. Kemp, O. Kemularia, Y. Kermaidic, W. Ketchum, S. H. Kettell, M. Khabibullin, N. Khan, A. Khvedelidze, D. Kim, J. Kim, M. J. Kim, B. King, B. Kirby, M. Kirby, A. Kish, J. Klein, J. Kleykamp, A. Klustova, T. Kobilarcik, L. Koch, K. Koehler, L. W. Koerner, D. H. Koh, L. Kolupaeva, D. Korablev, M. Kordosky, T. Kosc, U. Kose, V. A. Kosteleck\'y, K. Kothekar, I. Kotler, M. Kovalcuk, V. Kozhukalov, W. Krah, R. Kralik, M. Kramer, L. Kreczko, F. Krennrich, I. Kreslo, T. Kroupova, S. Kubota, M. Kubu, Y. Kudenko, V. A. Kudryavtsev, G. Kufatty, S. Kuhlmann, S. Kulagin, J. Kumar, P. Kumar, S. Kumaran, J. Kunzmann, R. Kuravi, N. Kurita, C. Kuruppu, V. Kus, T. Kutter, J. Kvasnicka, T. Labree, T. Lackey, I. Lal{\u{a}}u, A. Lambert, B. J. Land, C. E. Lane, N. Lane, K. Lang, T. Langford, M. Langstaff, F. Lanni, O. Lantwin, J. Larkin, P. Lasorak, D. Last, A. Laudrain, A. Laundrie, G. Laurenti, E. Lavaut, P. Laycock, I. Lazanu, R. LaZur, M. Lazzaroni, T. Le, S. Leardini, J. Learned, T. LeCompte, V. Legin, G. Lehmann Miotto, R. Lehnert, M. A. Leigui de Oliveira, M. Leitner, D. Leon Silverio, L. M. Lepin, J.-Y~Li, S. W. Li, Y. Li, H. Liao, C. S. Lin, D. Lindebaum, S. Linden, R. A. Lineros, A. Lister, B. R. Littlejohn, H. Liu, J. Liu, Y. Liu, S. Lockwitz, M. Lokajicek, I. Lomidze, K. Long, T. V. Lopes, J.Lopez, I. L{\'o}pez de Rego, N. L{\'o}pez-March, T. Lord, J. M. LoSecco, W. C. Louis, A. Lozano Sanchez, X.-G. Lu, K.B. Luk, B. Lunday, X. Luo, E. Luppi, D. MacFarlane, A. A. Machado, P. Machado, C. T. Macias, J. R. Macier, M. MacMahon, A. Maddalena, A. Madera, P. Madigan, S. Magill, C. Magueur, K. Mahn, A. Maio, A. Major, K. Majumdar, S. Mameli, M. Man, R. C. Mandujano, J. Maneira, S. Manly, A. Mann, K. Manolopoulos, M. Manrique Plata, S. Manthey Corchado, V. N. Manyam, M. Marchan, A. Marchionni, W. Marciano, D. Marfatia, C. Mariani, J. Maricic, F. Marinho, A. D. Marino, T. Markiewicz, F. Das Chagas Marques, C. Marquet, M. Marshak, C. M. Marshall, J. Marshall, L. Martina, J. Mart{\'\i}n-Albo, N. Martinez, D.A. Martinez Caicedo , F. Mart{\'i}nez L{\'o}pez, P. Mart\'inez Mirav\'e, S. Martynenko, V. Mascagna, C. Massari, A. Mastbaum, F. Matichard, S. Matsuno, G. Matteucci, J. Matthews, C. Mauger, N. Mauri, K. Mavrokoridis, I. Mawby, R. Mazza, T. McAskill, N. McConkey, K. S. McFarland, C. McGrew, A. McNab, L. Meazza, V. C. N. Meddage, A. Mefodiev, B. Mehta, P. Mehta, P. Melas, O. Mena, H. Mendez, P. Mendez, D. P. M{\'e}ndez, A. Menegolli, G. Meng, A. C. E. A. Mercuri, A. Meregaglia, M. D. Messier, S. Metallo, W. Metcalf, M. Mewes, H. Meyer, T. Miao, J. Micallef, A. Miccoli, G. Michna, R. Milincic, F. Miller, G. Miller, W. Miller, O. Mineev, A. Minotti, L. Miralles, C. Mironov, S. Miryala, S. Miscetti, C. S. Mishra, P. Mishra, S. R. Mishra, A. Mislivec, M. Mitchell, D. Mladenov, I. Mocioiu, A. Mogan, N. Moggi, R. Mohanta, T. A. Mohayai, N. Mokhov, J. Molina, L. Molina Bueno, E. Montagna, A. Montanari, C. Montanari, D. Montanari, D. Montanino, L. M. Monta{\~n}o Zetina, M. Mooney, A. F. Moor, Z. Moore, D. Moreno, O. Moreno-Palacios, L. Morescalchi, D. Moretti, R. Moretti, C. Morris, C. Mossey, C. A. Moura, G. Mouster, W. Mu, L. Mualem, J. Mueller, M. Muether, F. Muheim, A. Muir, Y. Mukhamejanov, M. Mulhearn, D. Munford, L. J. Munteanu, H. Muramatsu, J. Muraz, M. Murphy, T. Murphy, J. Muse, A. Mytilinaki, J. Nachtman, Y. Nagai, S. Nagu, R. Nandakumar, D. Naples, S. Narita, A. Navrer-Agasson, N. Nayak, M. Nebot-Guinot, A. Nehm, J. K. Nelson, O. Neogi, J. Nesbit, M. Nessi, D. Newbold, M. Newcomer, R. Nichol, F. Nicolas-Arnaldos, A. Nikolica, J. Nikolov, E. Niner, K. Nishimura, A. Norman, A. Norrick, P. Novella, A. Nowak, J. A. Nowak, M. Oberling, J. P. Ochoa-Ricoux, S. Oh, S.B. Oh, A. Olivier, A. Olshevskiy, T. Olson, Y. Onel, Y. Onishchuk, A. Oranday, M. Osbiston, J. A. Osorio V{\'e}lez, L. O'Sullivan, L. Otiniano Ormachea, J. Ott, L. Pagani, G. Palacio, O. Palamara, S. Palestini, J. M. Paley, M. Pallavicini, C. Palomares, S. Pan, P. Panda, W. Panduro Vazquez, E. Pantic, V. Paolone, R. Papaleo, A. Papanestis, D. Papoulias, S. Paramesvaran, A. Paris, S. Parke, E. Parozzi, S. Parsa, Z. Parsa, S. Parveen, M. Parvu, D. Pasciuto, S. Pascoli, L. Pasqualini, J. Pasternak, C. Patrick, L. Patrizii, R. B. Patterson, T. Patzak, A. Paudel, L. Paulucci, Z. Pavlovic, G. Pawloski, D. Payne, V. Pec, E. Pedreschi, S. J. M. Peeters, W. Pellico, A. Pena Perez, E. Pennacchio, A. Penzo, O. L. G. Peres, Y. F. Perez Gonzalez, L. P{\'e}rez-Molina, C. Pernas, J. Perry, D. Pershey, G. Pessina, G. Petrillo, C. Petta, R. Petti, M. Pfaff, V. Pia, L. Pickering, F. Pietropaolo, V.L.Pimentel, G. Pinaroli, S. Pincha, J. Pinchault, K. Pitts, K. Plows, C. Pollack, T. Pollman, F. Pompa, X. Pons, N. Poonthottathil, V. Popov, F. Poppi, J. Porter, L. G. Porto Paix{\~a}o, M. Potekhin, R. Potenza, M. Pozzato, T. Prakash, C. Pratt, M. Prest, F. Psihas, D. Pugnere, X. Qian, J. Queen, J. L. Raaf, V. Radeka, J. Rademacker, B. Radics, F. Raffaelli, A. Rafique, E. Raguzin, U. Rahaman, M. Rai, S. Rajagopalan, M. Rajaoalisoa, I. Rakhno, L. Rakotondravohitra, L. Ralte, M. A. Ramirez Delgado, B. Ramson, A. Rappoldi, G. Raselli, P. Ratoff, R. Ray, H. Razafinime, R. F. Razakamiandra, E. M. Rea, J. S. Real, B. Rebel, R. Rechenmacher, J. Reichenbacher, S. D. Reitzner, H. Rejeb Sfar, E. Renner, A. Renshaw, S. Rescia, F. Resnati, Diego~Restrepo, C. Reynolds, M. Ribas, S. Riboldi, C. Riccio, G. Riccobene, J. S. Ricol, M. Rigan, E. V. Rinc{\'o}n, A. Ritchie-Yates, S. Ritter, D. Rivera, R. Rivera, A. Robert, J. L. Rocabado Rocha, L. Rochester, M. Roda, P. Rodrigues, M. J. Rodriguez Alonso, J. Rodriguez Rondon, S. Rosauro-Alcaraz, P. Rosier, D. Ross, M. Rossella, M. Rossi, M. Ross-Lonergan, N. Roy, P. Roy, C. Rubbia, A. Ruggeri, G. Ruiz Ferreira, B. Russell, D. Ruterbories, A. Rybnikov, S. Sacerdoti, S. Saha, S. K. Sahoo, N. Sahu, P. Sala, N. Samios, O. Samoylov, M. C. Sanchez, A. S{\'a}nchez Bravo, A. S{\'a}nchez-Castillo, P. Sanchez-Lucas, V. Sandberg, D. A. Sanders, S. Sanfilippo, D. Sankey, D. Santoro, N. Saoulidou, P. Sapienza, C. Sarasty, I. Sarcevic, I. Sarra, G. Savage, V. Savinov, G. Scanavini, A. Scaramelli, A. Scarff, T. Schefke, H. Schellman, S. Schifano, P. Schlabach, D. Schmitz, A. W. Schneider, K. Scholberg, A. Schukraft, B. Schuld, A. Segade, E. Segreto, A. Selyunin, A. Selyunin, D. Senadheera, C. R. Senise, J. Sensenig, M. H. Shaevitz, P. Shanahan, P. Sharma, R. Kumar, S. Sharma Poudel, K. Shaw, T. Shaw, K. Shchablo, J. Shen, C. Shepherd-Themistocleous, A. Sheshukov, J. Shi, W. Shi, S. Shin, S. Shivakoti, I. Shoemaker, D. Shooltz, R. Shrock, B. Siddi, M. Siden, J. Silber, L. Simard, J. Sinclair, G. Sinev, Jaydip Singh, J. Singh, L. Singh, P. Singh, V. Singh, S. Singh Chauhan, R. Sipos, C. Sironneau, G. Sirri, K. Siyeon, K. Skarpaas, J. Smedley, E. Smith, J. Smith, P. Smith, J. Smolik, M. Smy, M. Snape, E.L. Snider, P. Snopok, D. Snowden-Ifft, M. Soares Nunes, H. Sobel, M. Soderberg, S. Sokolov, C. J. Solano Salinas, S. S\"oldner-Rembold, N. Solomey, V. Solovov, W. E. Sondheim, M. Sorel, A. Sotnikov, J. Soto-Oton, A. Sousa, K. Soustruznik, F. Spinella, J. Spitz, N. J. C. Spooner, K. Spurgeon, D. Stalder, M. Stancari, L. Stanco, J. Steenis, R. Stein, H. M. Steiner, A. F. Steklain Lisb\^oa, A. Stepanova, J. Stewart, B. Stillwell, J. Stock, F. Stocker, T. Stokes, M. Strait, T. Strauss, L. Strigari, A. Stuart, J. G. Suarez, J. Subash, A. Surdo, L. Suter, C. M. Sutera, K. Sutton, Y. Suvorov, R. Svoboda, S. K. Swain, B. Szczerbinska, A. M. Szelc, A. Sztuc, A. Taffara, N. Talukdar, J. Tamara, H. A. Tanaka, S. Tang, N. Taniuchi, A. M. Tapia Casanova, B. Tapia Oregui, A. Tapper, S. Tariq, E. Tarpara, E. Tatar, R. Tayloe, D. Tedeschi, A. M. Teklu, J. Tena Vidal, P. Tennessen, M. Tenti, K. Terao, F. Terranova, G. Testera, T. Thakore, A. Thea, S. Thomas, A. Thompson, C. Thorn, S. C. Timm, E. Tiras, V. Tishchenko, S. Tiwari, N. Todorovi{\'c}, L. Tomassetti, A. Tonazzo, D. Torbunov, M. Torti, M. Tortola, F. Tortorici, N. Tosi, D. Totani, M. Toups, C. Touramanis, D. Tran, R. Travaglini, J. Trevor, E. Triller, S. Trilov, J. Truchon, D. Truncali, W. H. Trzaska, Y. Tsai, Y.-T. Tsai, Z. Tsamalaidze, K. V. Tsang, N. Tsverava, S. Z. Tu, S. Tufanli, C. Tunnell, S. Turnberg, J. Turner, M. Tuzi, J. Tyler, E. Tyley, M. Tzanov, M. A. Uchida, J. Ure{\~n}a Gonz{\'a}lez, J. Urheim, T. Usher, H. Utaegbulam, S. Uzunyan, M. R. Vagins, P. Vahle, S. Valder, G. A. Valdiviesso, E. Valencia, R. Valentim, Z. Vallari, E. Vallazza, J. W. F. Valle, R. Van Berg, R. G. Van de Water, D. V.  Forero, A. Vannozzi, M. Van Nuland-Troost, F. Varanini, D. Vargas Oliva, S. Vasina, N. Vaughan, K. Vaziri, A. V{\'a}zquez-Ramos, J. Vega, S. Ventura, A. Verdugo, S. Vergani, M. Verzocchi, K. Vetter, M. Vicenzi, H. Vieira de Souza, C. Vignoli, C. Vilela, E. Villa, S. Viola, B. Viren, R. Vizarreta, A. P. Vizcaya Hernandez, Q. Vuong, A. V. Waldron, M. Wallbank, J. Walsh, T. Walton, H. Wang, J. Wang, L. Wang, M.H.L.S. Wang, X. Wang, Y. Wang, K. Warburton, D. Warner, L. Warsame, M.O. Wascko, D. Waters, A. Watson, K. Wawrowska, A. Weber, C. M. Weber, M. Weber, H. Wei, A. Weinstein, S. Westerdale, M. Wetstein, K. Whalen, A. White, A. White, L. H. Whitehead, D. Whittington, J. Wilhlemi, M. J. Wilking, A. Wilkinson, C. Wilkinson, F. Wilson, R. J. Wilson, P. Winter, W. Wisniewski, J. Wolcott, J. Wolfs, T. Wongjirad, A. Wood, K. Wood, E. Worcester, M. Worcester, M. Wospakrik, K. Wresilo, C. Wret, S. Wu, W. Wu, W. Wu, M. Wurm, J. Wyenberg, Y. Xiao, I. Xiotidis, B. Yaeggy, N. Yahlali, E. Yandel, J. Yang, K. Yang, T. Yang, A. Yankelevich, N. Yershov, K. Yonehara, T. Young, B. Yu, H. Yu, J. Yu, Y. Yu, W. Yuan, R. Zaki, J. Zalesak, L. Zambelli, B. Zamorano, A. Zani, O. Zapata, L. Zazueta, G. P. Zeller, J. Zennamo, K. Zeug, C. Zhang, S. Zhang, M. Zhao, E. Zhivun, E. D. Zimmerman, S. Zucchelli, J. Zuklin, V. Zutshi, R. Zwaska

